Model-agnostic bias mitigation methods with regressor distribution control for Wasserstein-based fairness metrics

This article is a companion paper to our earlier work Miroshnikov et al. (2021) on fairness interpretability, which introduces bias explanations. In the current work, we propose a bias mitigation methodology based upon the construction of post-processed models with fairer regressor distributions for Wasserstein-based fairness metrics. By identifying the list of predictors contributing the most to the bias, we reduce the dimensionality of the problem by mitigating the bias originating from those predictors. The post-processing methodology involves reshaping the predictor distributions by balancing the positive and negative bias explanations and allows for the regressor bias to decrease. We design an algorithm that uses Bayesian optimization to construct the bias-performance efficient frontier over the family of post-processed models, from which an optimal model is selected. Our novel methodology performs optimization in low-dimensional spaces and avoids expensive model retraining.

==> declarations.tex <==

\section*{Declarations}

\subsection*{Funding} Not applicable.

\subsection*{Conflicts of interest/Competing interests} Not applicable.

\subsection*{Ethics approval} Not applicable.

\subsection*{Consent to participate} Not applicable.

\subsection*{Consent for publication}
Not applicable.

\subsection*{Availability of data and material}
All data in the examples of the article are synthetic. In each example, we provide the explicit formulas for the joint data distribution.

\subsection*{Code availability.} Algorithm $1$ in Section \ref{sec::bias_mitigation} is at the core of the methodology. Since the code of Algorithm $1$ is the intellectual property of Discover Financial Services, we provide the list of publicly available Python packages for its implementation. Specifically, we use the package \texttt{sklearn.ensemble} for training a model, the package \texttt{numpy.random} for generating random parameters and the joint distribution of synthetic data, \texttt{sklearn.metrics} for computing performance metrics, \texttt{empirical\_distribution.ECDF} from the packge \texttt{statsmodels.distributions} for computing the Wasserstein and KS distances,  the package \texttt{bayesian-optimization} for Bayesian iterations. We believe Algorithm $1$ with the provided description can be easily reproduced.

\subsection*{Authors' contributions} Not applicable.

